A New Beam Polarimeter at COSY to Search for Electric Dipole Moments of Charged Particles

A calorimetric polarimeter based on inorganic LYSO scintillators is described. It has been designed for use in a storage ring to search for electric dipole moments (EDM) of charged particles such as the proton and deuteron. Its development and first use was on the Cooler Synchrotron (COSY) at the Forschungszentrum J\"ulich with 0.97 GeV/c polarized deuterons, a particle and energy suitable for an EDM search. The search requires a polarimeter with high efficiency, large analyzing power, and stable operating characteristics. With typical beam momenta of about 1 GeV/c, the scattering of protons or deuterons from a carbon target into forward angles becomes a nearly optimal choice of an analyzing reaction. The polarimeter described here consists of 52 LYSO detector modules, arranged in 4 symmetric blocks (up, down, left, right) for energy determination behind plastic scintillators for particle identification via energy loss. The commissioning results of the current setup demonstrate that the polarimeter is ready to be employed in a first direct search for an EDM on the deuteron, which is planned at COSY in the next two years.

==> paper/CHANGELOG.tex <==

% file ; line number ; date ; author 

% file: LYSO.tex modules.tex beam-tests.tex summary.tex
%------------------------------------------------------------

LYSO.tex 

